AdvDMD: Adversarial Reward Meets DMD For High-Quality Few-Step Generation

Diffusion models offer superior generation quality at the expense of extensive sampling steps. Distillation methods, with Distribution Matching Distillation (DMD) as a popular example, can mitigate this issue, but performance degradation remains pronounced when sampling steps are limited. Reinforcement learning (RL) has been leveraged to improve the few-step generation quality during distillation, with the potential to even surpass the performance of the teacher model. However, existing approaches are combinatorial in nature, merely integrating an RL process with the distillation process, which introduces unnecessary complexities. To address this gap, we propose AdvDMD, a method that seamlessly unifies DMD distillation and RL. Specifically, AdvDMD employs the adversarially trained discriminator from DMD2 as the reward model, which assigns low scores to generated images and high scores to real ones. It is trained on both intermediate and final states of the denoising process and updated online with the distilled model, enabling a holistic supervision of the sampling trajectories and mitigating reward hacking. We adopt a unified SDE backward simulation and a different training schedule for DMD and RL to enable a more stable and efficient training. Experimental results demonstrate that the 4-step AdvDMD outperforms the original 40-step model for SD3.5 on DPG-Bench, while achieving significant performance gains for SD3 on the GenEval. On Qwen-Image, our 2-step AdvDMD achieves superior performance over TwinFlow.

==> sections/apdx0_proofs.tex <==
\section{Proofs}

This is a placeholder for the proofs.

==> sections/sec0_intro.tex <==
\section{Introduction}

Flash Attention~\cite{dao2022flashattentionfastmemoryefficientexact} is a fast and memory-efficient attention mechanism for large language models. It is based on the idea of using a combination of a key-value cache and a lookup table to store the key-value pairs. This allows for a significant reduction in the number of memory accesses, which is especially important for large language models.
